Analyzing the impact of SARS-CoV-2 variants on respiratory sound signals

The COVID-19 outbreak resulted in multiple waves of infections that have been associated with different SARS-CoV-2 variants. Studies have reported differential impact of the variants on respiratory health of patients. We explore whether acoustic signals, collected from COVID-19 subjects, show computationally distinguishable acoustic patterns suggesting a possibility to predict the underlying virus variant. We analyze the Coswara dataset which is collected from three subject pools, namely, i) healthy, ii) COVID-19 subjects recorded during the delta variant dominant period, and iii) data from COVID-19 subjects recorded during the omicron surge. Our findings suggest that multiple sound categories, such as cough, breathing, and speech, indicate significant acoustic feature differences when comparing COVID-19 subjects with omicron and delta variants. The classification areas-under-the-curve are significantly above chance for differentiating subjects infected by omicron from those infected by delta. Using a score fusion from multiple sound categories, we obtained an area-under-the-curve of 89% and 52.4% sensitivity at 95% specificity. Additionally, a hierarchical three class approach was used to classify the acoustic data into healthy and COVID-19 positive, and further COVID-19 subjects into delta and omicron variants providing high level of 3-class classification accuracy. These results suggest new ways for designing sound based COVID-19 diagnosis approaches.

==> table_old_sound_categories.tex <==
\begin{table*}[]
\rowcolors{2}{white}{gray!10}
\begin{tabular}{p{2.5cm}|p{13.5cm}}
\hline
\rowcolor[HTML]{9B9B9B} 
\textbf{Stimulus} & \textbf{Remarks} \\ \hline
breathing deep, breathing shallow         &  Breathing sound involves respiratory tract, lungs etc. It may contain COVID-19 bio-marker as it affects lungs. Breathing deep is produced by more respiratory effort.\\ \hline
cough heavy, cough shallow          & Cough production uses respiratory tract, glottis, lungs etc. It may contain COVID-19 bio-marker if it is present in voicebox. Coughing heavily requires more involvement of lower respiratory organs.\\ \hline
    vowel a, vowel e and vowel o        &  These are sustained phonation of three different vowels. They involve vocal tract, tongue, oral cavity etc. They may contain COVID-19 bio-marker if it has effect on vowel formant frequencies. \\ \hline
    counting fast and counting normal            & It is the counting of digits from 1 to 20. Complete voice production and associated system is involved in this sound. It may contain COVID-19 signature that is not captured in above categories because speech is more complicated sound\\ \hline
\end{tabular}
\caption{Stimulus categories and their significance}
\label{resp_table}
\end{table*}

==> table_subject_categories.tex <==
\begin{table}[]
\centering
\rowcolors{2}{white}{gray!10}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Subject Category} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{Description}} \\ \midrule
Non-COVID &  & Not infected with COVID-19 \\
COVID-Pre-O &  & \begin{tabular}[c]{@{}l@{}}Infected with COVID-19 with\\ a strain earlier to Omicron outbreak\end{tabular} \\
COVID-O &  & \begin{tabular}[c]{@{}l@{}}Infected with COVID-19 with\\ a strain during Omicron outbreak\end{tabular} \\ \bottomrule
\end{tabular}
}
\caption{}
\label{tab:my-table}
\end{table}
